On Nesting Monte Carlo Estimators

Many problems in machine learning and statistics involve nested expectations and thus do not permit conventional Monte Carlo (MC) estimation. For such problems, one must nest estimators, such that terms in an outer estimator themselves involve calculation of a separate, nested, estimation. We investigate the statistical implications of nesting MC estimators, including cases of multiple levels of nesting, and establish the conditions under which they converge. We derive corresponding rates of convergence and provide empirical evidence that these rates are observed in practice. We further establish a number of pitfalls that can arise from naive nesting of MC estimators, provide guidelines about how these can be avoided, and lay out novel methods for reformulating certain classes of nested expectation problems into single expectations, leading to improved convergence rates. We demonstrate the applicability of our work by using our results to develop a new estimator for discrete Bayesian experimental design problems and derive error bounds for a class of variational objectives.

==> bias_proof.tex <==
% !TEX root =  main.tex

\section{Proof for Theorem~\ref{the:bias} - Lack of General Purpose Unbiased Estimator}
\label{sec:app:bias-proof}

\theBias*

\begin{proof}
	Take $f(y, w) = (\gamma(y) - w)^2$. Then $f(y, \gamma(y)) = 0$, so that $I(f) = 0$.  On
	the other hand, $f(y_n, \hat{\zeta}_n) \geq 0$ since $f$ is non-negative.
	Moreover, $f(y_n, \hat{\zeta}_n) > 0$ on the event $\{\hat{\zeta}_n \neq \gamma(y_n)\}$.
	Since we assumed this event has nonzero probability, it follows that $\E \left[f(y_n, \hat{\zeta}_n)\right] > 0$ and hence
	\[
	\E\left[\frac{1}{N} \sum_{n=1}^N f(y_n, \hat{\zeta}_n)\right]
	= \frac{1}{N} \sum_{n=1}^N \E\left[f(y_n, \hat{\zeta}_n)\right]
	> 0 = I(f)
	\]
	which gives the required result.
\end{proof}

==> convex.tex <==
% !TEX root =  main.tex

\section{Proof of Bias for Convex or Concave Functions}
\label{sec:app:convex}

\begin{theorem}
	\label{the:bias-conv}	
	Suppose that $y_n \sim p(y)$ and that each $\hat{\zeta}_n$ satisfies $\E \left[\hat{\zeta}_n \middle| y_n\right] = \gamma(y_n)$.
	Define $\mathcal{A} \subseteq \mathcal{Y}$ as
	$\mathcal{A} = \left\{y \in \mathcal{Y} \;\middle|\; \mathrm{Var}\left(\hat{\zeta}_n \middle| y_n=y \right)>0\right\}$
	and assume that ~$\mathbb{P}(y_n \in \mathcal{A}) > 0$.
	Then for any $f$ that is strictly convex in its second argument,
	\[ 
	\E\left[\frac{1}{N} \sum_{n=1}^N f(y_n, \hat{\zeta}_n)\right] > I(f).
	\]
	Similarly for any $f$ that is strictly concave in its second argument, 
	\[
	\E\left[\frac{1}{N} \sum_{n=1}^N f(y_n, \hat{\zeta}_n)\right] < I(f).
	\]
\end{theorem}
\begin{proof}
	We prove our claim for the case that $f$ is strictly convex; our proof for the other concave case  
	is symmetrical. We have
	\begin{align*}
	\E\left[\frac{1}{N} \sum_{n=1}^N f(y_n, \hat{\zeta}_n)\right] = \E\left[f(y_1, \hat{\zeta}_1)\right]
	= \E\left[\E\left[f(y_1, \hat{\zeta}_1) \middle| y_1\right]\right] 
	\ge \E\left[f\left(y_1, \E\left[\hat{\zeta}_1 \middle| y_1\right]\right)\right] = I(f)
	%        \E&\left[\frac{1}{N} \sum_{n=1}^N f(y_n, \hat{\zeta}_n)\right] = \E\left[f(y_1, \hat{\zeta}_1)\right] \\
	%        & \quad \quad \quad \quad = \E\left[\E\left[f(y_1, \hat{\zeta}_1)|y_1\right]\right] \\
	%        & \quad \quad \quad \quad = \E\left[\mathbb{I}(y_1 \in \mathcal{A}) \E\left[f(y_1, \hat{\zeta}_1)|y_1\right]\right] \\
	%        & \quad \quad \quad \quad \quad + \E\left[\mathbb{I}(y_1 \notin \mathcal{A}) \E\left[f(y_1, \hat{\zeta}_1)|y_1\right]\right] \\
	%        & \quad \quad \quad \quad \ge \E\left[\mathbb{I}(y_1 \in \mathcal{A}) f\left(y_1, \E\left[\hat{\zeta}_1 \middle| y_1\right]\right)\right] \\
	%        & \quad \quad \quad \quad \quad + \E\left[\mathbb{I}(y_1 \notin \mathcal{A}) \E\left[f(y_1, \hat{\zeta}_1)|y_1\right]\right] \\    
	%        & \quad \quad \quad \quad = \E\left[\E\left[f(y_1, \hat{\zeta}_1)|y_1\right]\right] = I(f)
	\end{align*}
	where the $\ge$ is a result of Jensen's inequality on the inner expectation.  
	Since $f$ is strictly convex and therefore non-linear, equality holds if and only if
	$\hat{\zeta}_1$ is almost surely constant given $y_1$. 
	This is violated whenever $y_1 \in \mathcal{A}$, which by assumption
	has a non-zero probability of occurring.  Consequently,
	the inequality must be strict, giving the desired result.
\end{proof}

==> linear-proof.tex <==
% !TEX root =  supp.tex

\section{Proof for Theorem 1 - Convergence Rate for Finite Realisations of $y$}

Here we repeat Theorem 1 from the main paper and provide the full proof.

\begin{theorem}
	If $f$ is Lipschitz continuous, then the mean squared error of 
	\[
	I_N = \sum_{c=1}^C (\hat{P}_N)_c \, (\hat{f}_N)_c
	\]
	as an estimator for $I$ converges at rate $O(1/N)$.
\end{theorem}

\begin{proof}
	Denote
	\[
	P_c = P(y = y_c)
	\]
	and
	\[
	f_c = f(y_c, \gamma(y_c)).
	\]
	Then, Minkowski's inequality allows us to bound the mean squared error as
	\begin{eqnarray*}
		\E\left[(I_N - I)^2\right] &=& \norm{I_N - I}_2^2 \\
		&\leq& \left(\sum_{c=1}^C W_c \right)^2,
	\end{eqnarray*}
	where
	\[
	W_c := \norm{(\hat{P}_N)_c \, (\hat{f}_N)_c - P_c \, f_c}_2.
	\]
	Moreover, again by Minkowski, we have
	\[
	W_c \leq U_c + V_c
	\]
	where 
	\[
	U_c = \norm{(\hat{P}_N)_c \, (\hat{f}_N)_c - (\hat{P}_N)_c \, f_c}_2
	\]
	and
	\[
	V_c = \norm{(\hat{P}_N)_c \, f_c - P_c \, f_c}_2.
	\]
	Factoring out $(\hat{P}_N)_c$ in $U_c$ gives
	\begin{eqnarray*}
		U_c &=& \sqrt{\E\left[(\hat{P}_N)_c^2 \, \left((\hat{f}_N)_c - f_c\right)^2\right]} \\
		&=& \sqrt{\E\left[(\hat{P}_N)_c^2\right]} \sqrt{\E\left[\left((\hat{f}_N)_c - f_c\right)^2\right]},
	\end{eqnarray*}
	since we assume we sample each $y_n$ and $z_n$ independently. Using Minkowski's
	inequality, we may write the first right-hand term as
	\begin{eqnarray*}
		\sqrt{\E\left[(\hat{P}_N)_c^2\right]} &=& \norm{(\hat{P}_N)_c}_2 \\
		&\leq& \frac{1}{N} \sum_{n=1}^N \norm{\mathbbm{1}(y_n = y_c)}_2 \\
		&=& \frac{1}{N} \sum_{n=1}^N P_c = P_c.
	\end{eqnarray*}
	For the second term, note that by Lipschitz continuity, we have for some constant $K >
	0$
	\begin{eqnarray*}
		\sqrt{\E\left[\left((\hat{f}_N)_c - f_c\right)^2\right]} &=&
		\norm{(\hat{f}_N)_c - f_c}_2 \\
		&\leq& K \, \norm{\frac{1}{N} \sum_{n=1}^N \phi(y_c, z_n) - \gamma(y_c)}_2 \\
		&=& K \cdot O(1/\sqrt{N}) \\
		&=& O(1/\sqrt{N}),
	\end{eqnarray*}
	since $\frac{1}{N} \sum_{n=1}^N \phi(y_c, z_n)$ is a Monte Carlo estimator for
	$\gamma(y_c)$. Altogether then, we have that
	\[
	U_c = P_c \cdot O(1 / \sqrt{N}) = O(1 / \sqrt{N}).
	\]
	We can also factor out $f_c$ in $V_c$ to obtain
	\[
	V_c = |f_c| \cdot \norm{(\hat{P}_N)_c - P_c}_2 = |f_c| \cdot O(1/\sqrt{N}) = O(1/\sqrt{N}),
	\]
	since $(\hat{P}_N)_c$ is a Monte Carlo estimator for $P_c$.
	
	These asymptotic bounds for $U_c$ and $V_c$ then entail that our overall mean squared
	error satisfies
	\begin{eqnarray}
	\E\left[(I_N - I)^2\right] &\leq& 2^{\lceil \log_2 C \rceil} \sum_{c=1}^C W_c^2 \label{eq:square-inequal-1} \\
	&\leq& 2^{\lceil \log_2 C \rceil} \sum_{c=1}^C (U_c + V_c)^2 \notag \\
	&\leq& 2^{\lceil \log_2 C \rceil + 1} \sum_{c=1}^C U_c^2 + V_c^2 \label{eq:square-inequal-2} \\
	&=& 2^{\lceil \log_2 C \rceil + 1} \sum_{c=1}^C O(1/N) + O(1/N) \notag \\
	&=& O(1/N), \notag
	\end{eqnarray}
	as desired. Note that in \eqref{eq:square-inequal-1} and
	\eqref{eq:square-inequal-2} we have used the fact that
	\[
	\left(\sum_{\ell=1}^L A_\ell\right)^2 \leq 2^{\lceil \log_2 L \rceil} \sum_{\ell=1}^L A_\ell^2
	\]
  for all $A_1, \cdots, A_L \in \mathbb{R}$, which itself follows by an inductive argument
  from the fact that
	\[
    (A+B)^2 \le 2(A^2+B^2)
	\]	
	for any $A, B \in \mathbb{R}$.
\end{proof}


==> probprog.tex <==
% !TEX root =  main.tex

\section{Nesting Probabilistic Programs}
\label{sec:probprog}

Probabilistic programming systems (PPSs) allow probabilistic models to be represented in the 
form of a generative model and statements for conditioning on data~\citep{goodman2008church,gordon2014probabilistic}.
Informally, one can think of the generative model as the definition of a prior, the conditioning 
statements as the definition of a likelihood, and the output of the program as samples from a posterior distribution. 
Their core philosophy is to decouple model specification and inference, the former 
corresponding to the user-specified program code and the latter to an inference engine 
capable of operating on arbitrary programs.  Removing the need for users to write 
inference algorithms significantly reduces the burden of developing new models and 
makes effective statistical methods accessible to non-experts.  

Some, so-called universal, systems~\cite{goodman2008church,goodman_book_2014,mansinghka2014venture,wood2014new} 
further allow the definition of models that would be hard, or
even impossible, to convey using conventional frameworks such as graphical models.
One enticing manner they do this is by allowing
arbitrary nesting of models, known in the probabilistic programming literature as queries~\citep{goodman2008church},
such that it is easy to define and run nested inference 
problems~\citep{goodman2008church,mantadelis2011nesting,stuhlmuller2014reasoning}. 
This allows the definition of models that could not be encoded without nesting, such as those involving
agents reasoning about other agents~\cite{le2016nested} and experimental design problems~\cite{ouyang2016practical}.
For example, one might use such nesting to model a poker player reasoning about another player as shown
in Appendix~\ref{sec:poker}. See also~\cite{stuhlmuller2014reasoning} for a number of other examples.

The aim of this section is to establish the implications of our NMC results on the statistical correctness of
nesting probabilistic program queries.  We consider different ways one might nest queries
and assess their respective correctness.  Namely, we consider \emph{sampling} from the conditional distribution
of another query, \emph{observing} another query, and using \emph{estimates as variables}
in another query.  We further outline some special cases where standard \mc convergence can be achieved.
We will use \emph{Anglican}~\citep{tolpin2016design,wood2014new} syntax
as a basis for discussion,
an introduction for which is provided in the next section, noting that our results apply more generally.  
We find that changes are required to how Anglican tackles nested query problems to
ensure consistency and allow exploitation of the special cases.  
%Empirical evidence supporting our theoretical
%discussions are provided in Appendices~\ref{sec:emp} and~\ref{sec:exp}.

% !TEX root = main.tex

\subsection{The Anglican Probabilistic Programming Language}
\label{sec:anglican}

Anglican is a universal PPL integrated into \emph{Clojure}~\citep{hickey2008clojure}, a dynamically-typed, general-purpose, functional
programming language (specifically a dialect of Lisp) that runs on the Java virtual machine and uses just-in-time compilation.
There are two key things to get your head around for reading and using Clojure (and Lisp languages more
generally): almost everything is a function and parentheses evaluate functions.  For example, to code $a+b$ in Clojure one
would write {\small \lsi{(+ a b)}} where \clj{+} is a function taking two arguments (here \clj{a} and \clj{b}) and the parentheses cause the
function to evaluate.  More generally, Clojure uses prefix notation such that 
the first term in a parenthesis is always a function, with the other terms the arguments.
Thus {\small \lsi{((+ a b))}} would be invalid syntax as the result of {\small \lsi{(+ a b)}}  is not a function so cannot be evaluated.
Expressions are nested in a tree structure so to code $2(a+b)/c$ one would write {\small \lsi{(/ (* 2 (+ a b)) c)}}.  One can
thus think about going outwards in terms of execution order -- a function first evaluates its arguments before
itself.  Functions in Clojure are first class (i.e. they can be variables) and can be declared either anonymously using
{\small \lsi{(fn [args] body)}}, for example {\small \lsi{(fn [a b] (/ a b))}}, or using the
macro \defn to declare a named function in the namespace, for example {\small \lsi{(defn divide [a b] (/ a b))}}.
Local bindings in Clojure are defined using \cllet blocks which denote a number of name-value pairs for
binding variables, followed by a series of evaluations to  carry out. Their return value
is the output of the last of these evaluations.  Thus for example
{\small \lsi{(let [a 2 b 3] (print a) (+ a b))}} says let $a$ be equal to $2$, $b$ be equal to $3$, print $a$,
and then evaluate $a+b$, thus returning $5$.  

Anglican inherits most of the syntax of Clojure, but extends it with the key
special forms \sample and \observe \citep{tolpin2015probabilistic,tolpin2016design}, between which the distribution of the
query is defined. 
Informally, \sample specifies terms in the prior and \observe terms in the
likelihood.  More precisely, \sample is used to make random draws $x_t \sim f_t(x_t | \Xi_t)$,
where $\Xi_t$ is a subset of the variables in scope at the point of sampling, and \observe is used to condition on
data $g_s(y_s|\Lambda_s)$ with $\Lambda_s$ defined in the same way as $\Xi_t$.  
The syntax of \sample is to take a \emph{distribution object} as its only input, while \observe
takes a distribution object and an observation as input.  Each distribution
object further contains a sampling procedure and a density function.  
Anglican provides a number of \emph{elementary random procedures} in
the form of distribution classes for common sampling distributions such as the normal and Poisson
distributions, but also allows users to define their own distribution classes using the \defdist macro.
Distribution objects are generated by calling the class constructor
with the required parameters, e.g. {\small \lsi{(normal 0 1)}} for the unit Gaussian.
Despite using predominantly the same syntax, Anglican has different
\emph{probabilistic} semantics to Clojure, i.e. code is written in the same way, but is interpreted differently.

\begin{wrapfigure}{r}{0.35\textwidth}
	\centering 
	\vspace{-10pt}
	\begin{lstlisting}[basicstyle=\ttfamily\small]
(defquery my-query [data]
 (let [mu (sample (normal 0 1))
       sig (sample (gamma 2 2))
       lik (normal mu sig)]
  (map (fn [obs]
   (observe lik obs))
   data)
  [mu sig]))
	\end{lstlisting}	
	\vspace{-5pt}
	\caption{A simple Anglican query.\label{fig:probprog:simple-ang}}
	\vspace{-5pt}
\end{wrapfigure}
Anglican queries are written using the macro \defquery.  This allows users to define a model using a mixture
of \sample and \observe statements and deterministic code, and bind that model to a variable.  
A simple example of an Anglican query is shown in Figure~\ref{fig:probprog:simple-ang},
corresponding to a model where we are trying to infer the mean and standard deviation
of a Gaussian given some data.  The syntax of \defquery is {\small \lsi{(defquery name [args] body)}}
so in Figure~\ref{fig:probprog:simple-ang} our query is named {\small \lsi{my-query}} and takes
in arguments {\small \lsi{data}}.  The query starts by sampling {\small \lsi{mu}}$\sim\mathcal{N}(0,1)$
and {\small \lsi{sig}}$\sim\textsc{Gamma}(2,2)$ and constructing a distribution object {\small \lsi{lik}}
to use for the observations.  It then maps over each datapoint and observes it under the distribution
{\small \lsi{lik}}, remembering that {\small \lsi{fn}} defines a function and \map applies a function
to every element of a list or vector.  
Note that \observe simply returns {\small \lsi{nil}} and so we
are not interested in these outputs -- they affect the probability of a program execution trace, but
not the calculation of a trace itself.  After the observations are made, {\small \lsi{mu}} and {\small \lsi{sig}}
are returned from the \cllet block and then by proxy the query itself.
This particular query defines a correctly normalized joint distribution (note some queries are not normalized) given by
\begin{align}
p(\mu,\sigma,y_{1:S}) = \mathcal{N}(\mu ; 0,1) \; \textsc{Gamma}(\sigma ; 2, 2) \prod_{s=1}^{S} \mathcal{N}(y_s ; \mu, \sigma)
\end{align}
where we have defined $\mu:=${\small \lsi{mu}}, $\sigma:=${\small \lsi{sig}}, and $y_{1:S}:=${\small \lsi{data}}.

Inference on a query is performed using the macro \doquery, which produces a lazy infinite sequence of 
approximate samples from the conditional distribution and, for appropriate inference algorithms,
an estimate of the partition function.
The syntax of \doquery is {\small \lsi{(doquery inf-alg model inputs & options)}} where {\small \lsi{inf-alg}}
specifies an inference algorithm, {\small \lsi{model}} is our query, {\small \lsi{inputs}}
is a vector of inputs to the query, the \& represents that there might be multiple additional inputs, and {\small \lsi{options}}
is a series of option-value pairs for the inference engine.  For example, to produce 100 samples from
our {\small \lsi{my-query}} model with data {\small \lsi{[2.1 5.2 1.1]}} using the LMH inference algorithm with no
additional options, we can write {\small \lsi{(take 100 (doquery :lmh my-query [2.1 5.2 1.1]))}}.

Although Anglican mostly inherits Clojure syntax, some complications arise from the compilation to
CPS-style Clojure functions, required for performing inference.  It is thus not possible to na\"{i}vely 
use all Clojure functions inside Anglican
without providing appropriate information to the compiler to perform the required transformation.
The transformation for many core Clojure functions has been coded manually, such that they form
part of the Anglican syntax and can be used directly.  Anglican further allows users to write functions externally
to \defquery using the macro \defm, which is analogous to \defn in Clojure and has the same call syntax,
which can then be called from inside the query without restrictions.  Other deterministic Clojure functions can also
be called from inside queries but must be provided with appropriate wrapping to assist the compiler.  Thankfully
this is done automatically (except when the function itself is higher order) using the macro
{\small \lsi{with-primitive-procedures}} that takes as inputs Clojure functions and creates an environment where
these functions have been converted to their appropriate CPS forms.

For our purposes, an important element of Anglican is its ability to \emph{nest} queries within one another.
Though \doquery is not allowed directly within a \defquery block, one can still nest queries by 
using the special form \conditional which
takes a query and returns a distribution object constructor ostensibly corresponding to the conditional distribution 
(informally the posterior) defined by the query, for which the inputs to the query become the parameters.  However,
our results show that the default use of \conditional does not have this interpretation in the nested query
context.  In truth, \conditional defines a Markov chain whose samples converge in distribution to the conditional
distribution defined by the query.  When using \conditional as an alternative to \doquery, this is not problematic
as estimates calculated using the outputs converge by the strong law of large numbers.  However, when used to nest
queries, this Markov chain is only ever run for a finite length of time (specifically one accept-reject step is
carried out) and so does
not produce samples from the true conditional distribution.  By default, this Markov chain is generated by equalizing
the output of sequence of importance samples (i.e. it is a Metropolis sampler using independent proposals).  However,
\conditional does allow the specification of an inference algorithm and associated options, which in the nested
query context leads to explicitly distinct distributions.  Though hardly its intended use, this does actually provide
a roundabout means of arbitrarily reducing the bias in Anglican's nested query inference (ignoring memory restrictions) using
\clj{(conditional inner-query :smc :number-of-particles N_k)} as each sample output by the SMC sweep convergences in
distribution to the conditional distribution as $N_k\to \infty$ (noting that as a resampling step is done at the end
of the sweep, all particles in a sweep have the same weight).

Though not officially supported usage, one can also nest Anglican queries by using a \doquery in a Clojure function 
that is then passed to another query using {\small \lsi{with-primitive-procedures}} or
using a \doquery within a custom distribution defined by \defdist.  This allows our ``estimates as variables'' class
of models to be encoded.


\subsection{Nested Sampling}
\label{sec:samp}

One of the clearest ways one might want to nest queries is by sampling from the conditional
distribution of one query inside another query.  A number of examples of this are provided
for Church in~\cite{stuhlmuller2014reasoning}.
%\footnote{Even though the nested calls are made inside the conditioning
%	predicate for these examples, the semantics of Church (in particular only using hard constraints) 
%	means these behave as per our definition of nesting sampling.}
Such problems fall under a more general framework of \emph{nested inference}~\citep{mantadelis2011nesting} or equivalently inference for so-called
\emph{doubly (or multiply) intractable} distributions~\citep{murray2006mcmc,stuhlmuller2014reasoning}.
The key feature of these problems is that they include
terms with unknown, \emph{parameter dependent}, normalization constants.  For nested probabilistic programming
queries, this is manifested in \emph{conditional normalization} within a query.
Consider as an example the following Anglican model using a nested calling structure
\vspace{-10pt}
\begin{lstlisting}[basicstyle=\ttfamily\footnotesize,multicols=2,frame=none]
(defm inner [y D]
 (let [z (sample (gamma y 1))]
  (observe (normal y z) D)
  z))

(defquery outer [D]
 (let [y (sample (beta 2 3))
       z (inner y D)]
  (* y z)))
\end{lstlisting}
\vspace{-24pt}
compared to the following nested query model
\vspace{-10pt}
\begin{lstlisting}[basicstyle=\ttfamily\footnotesize,multicols=2,frame=none]
(defquery inner [y D]
 (let [z (sample (gamma y 1))]
  (observe (normal z y) D)
  z))

(defquery outer [D]
 (let [y (sample (beta 2 3))
       dist (conditional inner)
       z (sample (dist y D))]
  (* y z)))
\end{lstlisting}
\vspace{-15pt}
where we have replaced the function deceleration \defm with a query nesting using
the \conditional special form.  The unnormalized distribution on
traces for the first model is straightforwardly given by
\[
\tilde{\pi}_1(z,y,D) = p(y)p(z|y)p(D|y,z) = \textsc{Beta}(y;2,3) \textsc{Gamma}(z;y,1) \mathcal{N}(D;z,y^2),
\]
for which we can use conventional Monte Carlo inference schemes.  The second model
differs in that $p(z|y)p(D|y,z)$ is conditionally normalized 
before being used in the outer query
\[
\tilde{\pi}_2(z,y,D) = p(y)p(z|y,D) = p(y)\frac{p(z|y)p(D|y,z)}{\int p(z|y)p(D|y,z)dz} = p(y)\frac{p(z|y)p(D|y,z)}{p(D|y)} \neq \tilde{\pi}_1(z,y,D).
\]
The key point here is that the partial normalization constant $p(D|y)$ depends on $y$ and so 
$\tilde{\pi}_2(z,y,D)$ is doubly intractable because we cannot evaluate our unnormalized target
distribution exactly.  By normalizing $p(z|y)p(D|y,z)$ within the outer query, 
\conditional has changed the distribution defined by the program.  Another interesting way of looking at this
is that wrapping \clj{inner} in \conditional has ``protected'' $y$ from the conditioning 
in \clj{inner} (noting
that $\tilde{\pi}_1 (z,y,D) \propto p(y|D)p(z|y,D)$) such that the \observe statement only affects the probability
of $z$ given $y$ and not the probability of $y$.

Given that this problem cannot be rearranged to a single expectation, it now obvious to ask the question: what behavior do we need for \conditional, or query nesting through sampling
more generally, in order to ensure consistency?  
%From a practical perspective, it becomes much easier to write programs which will never terminate
%as, using the notation from our previous example, then for all possible $y$, there must be some $z$
%for which $p(D|y,z)\neq0$ (or for which the condition holds true in the context of Church).
%WRONG!
%Imagine we take
%a rejection sampling approach whereby no sample ever returns until
%it passes the acceptance criterion (which seems to be the approach taken by Church).  One clear issues this throws up is that it might be the case
%that the inner query has no valid outputs for a particular input.  Using the notation from our earlier example, we
%might have that $p(z|y,D) = 0, \forall z$ for a particular value of $y$, e.g. if $p(D|y,z) = \mathbb{I}(|y|<1 \cap |z|<1)$
%then any $|y|\ge1$ outside this range has zero probability.  
%Our outer distribution here $\tilde{\pi}_2(z,y,D)$
%is still well defined, it just happens to be zero unless $|y|<1$.  Thus our depth-first rejection 
%strategy could get permanently stuck for a fundamentally computable distribution.  On the other hand,
%we could instead 
Without access to exact sampling methods, it follows from Theorem~\ref{the:Repeat} (and the nonlinear
mapping originating from the inversion of the normalization constant)
that asymptotic bias is, in general, unavoidable for
query nesting if each call of \conditional only carries out finite computation.
In other words, we need the computational budget of each \conditional call to 
become arbitrarily large for convergence.
%This follows from our general NMC results and
%the fact that normalization constitutes a nonlinear mapping.


\begin{figure*}[t!]
	\centering
	{\includegraphics[width=0.45\textwidth,trim={1.5cm 0 3.5cm 2cm},clip]{../Figures/prog_hists}}
		{\caption{Histograms showing a comparison of the output samples (i.e. of $z\times y$) produced by the nested Anglican
				queries given in the text to approximate ground truth reference,
				the ``unnested'' model,
				and a na\"{i}ve estimation scheme where $N_1=1$.\label{fig:hists}}}
	\vspace{-15pt}
\end{figure*}	

As an sanity check for this theoretical result, we conduct an empirical evaluation to
check that this behavior manifests in practice.  We ran Anglican's importance sampling inference
engine on the simple model introduced earlier and compared this to approximate ground truth reference code (implemented in 
\textsc{Matlab}) where each call to \clj{inner} internally generates $N_1=10^3$ samples before drawing the returned $z$ from these
in proportion to the weights, giving a close approximation to $p(z|y,D)$.
As shown in Figure~\ref{fig:hists}, the samples produced by Anglican are substantially different to
the reference code, demonstrating that the outputs do not match their semantically intended distribution.
For reference, we also consider the distribution induced by the ``unnested'' model, where \conditional is replaced
by \clj{defm}, and a na\"{i}ve estimation scheme where a sample budget of $N_1=1$ is used for each call
to \clj{inner}, effectively corresponding to ignoring the \observe statement by directly returning the
first draw of $z$.  We see that the unnested model defines a noticeably different distribution, while the behavior
of Anglican is similar, but distinct, to ignoring the \observe statement in the inner query.  Further
investigation shows that the default behavior of \conditional in a query nesting context is equivalent to the 
reference code but with $N_1=2$, inducing a substantial bias. 

A special case where consistency can be maintained without requiring infinite computation for each nested call
is when no
random variables are input to the inner query.  
A condition for this is that we use a method that provides an unbiased estimate of 
the partition function (e.g. sequential \mc (SMC)) and factor the trace weight appropriately
with the product of this partition function estimate and the internal self-normalized weight
of the returned sample.  
If this condition is maintained, we can demonstrate the validity of the approach by noting that
the normalization constant of the nested query is not parameter dependent, i.e. $p(D|y)=p(D)$ 
using the notation from our earlier example.  It can, therefore, 
be factored into the outer query: the nested query now defines the same distribution 
as if the conditional query were replaced with a standard function, e.g. \defm in Anglican.  We can thus view inference 
on such problems as taking a pseudo-marginal approach~\citep{andrieu2009pseudo,andrieu2010particle}, provided that all samples returned from
the inner query are properly weighted~\citep{naessethLS2015nested}.
The correctness of this approach then follows Theorem~\ref{the:prod}.
However, Anglican's current use of \conditional, for example, does not
satisfy our requirement as it only returns unweighted samples.
For Anglican to provide consistent estimates in such situations, one would need to
change the probabilistic semantics of \conditional, such that it
both produces a sample and simultaneously factors the outer query trace weight.
%In other words, it would need to operate in a similar fashion
%to the following simplified code
%\begin{lstlisting}[basicstyle=\ttfamily\footnotesize,frame=none]
%(defn conditional-sample [inner-query inputs inf-alg M inf-opts]
% (let [samp (nth M (doquery inf-alg inner-query inputs inf-opts))]
%  (observe (factor) (get-log-weight samp))
%  (:result samp)))
%\end{lstlisting}
%\vspace{-10pt}
%where we run inference with budget \texttt{M} to produce a sample, weight the program trace
%using the (unnormalized) sample weight, and return the value of the sample.
%Note that our special case corresponds to \clj{inputs} being deterministic
%and samples being properly weighted.  When this is not
%satisfied, it will be necessary for \texttt{M} to increase as more samples are produced
%to ensure consistency.

Another special case is when the variables passed to the inner query can only take on, say $C$, finite
possible values. This special case is one which requires rearrangement
or a specialist consideration by the language back-end (as done by e.g. \cite{cornish2017efficient,stuhlmuller2012dynamic,stuhlmuller2014reasoning}),
with na\"{i}ve implementations leading to NMC convergence rates.  It emphasizes that
nested problems with continuous variables are a fundamentally different problem
class to those with only bounded discrete variables (or only continuous variables at the bottom layer)
and we must, therefore, be wary of presuming that results from the discrete case carry over.


\subsubsection{Example Application -- Simulating a Poker Player}
\label{sec:poker}

As a more realistic demonstration of the utility for allowing nested query sampling
in probabilistic programs, we consider the example of simulating a poker player who reasons about
another player. Anglican code for this example is given in Figure~\ref{fig:poker-code}.
In the interest of exposition, we consider the simple situation where both players are short-stacked, such that player 1's (P1's)
only options are to fold or go all-in.  Presuming that P1 has bet, the second player (P2)
can then either fold or call. One could easily adapt
the model to consider multiple players and cases where the players have
more options than the binary choice of betting or not, including cases where the actions might be continuous,
and where there are multiple rounds of betting (for which addition levels to the nesting would be required).

\begin{figure}[p]
	\begin{lstlisting}[basicstyle=\ttfamily\footnotesize,frame=none]
(defdist factor [] []
 ;; Factors trace probability with provided value
 (sample* [this] nil)
 (observe* [this value] value))
	
(defdist hand-strength []
 ;; Samples the strength of a hand
 [dist (uniform-continuous 0 1)]
 (sample* [this] (sample* dist))
 (observe* [this value] (observe* dist value)))
	
(defdist play-prior [hand]
 ;; A prior on whether to play a hand without reasoning about the opponent
 [dist (categorical
        {:fold (+ 0.25 (* 0.75 (- 1. hand)))
         :bet (+ 0.25 (* 0.75 hand))})]
 (sample* [this] (sample* dist))
 (observe* [this value] (observe* dist value)))
	
(with-primitive-procedures [hand-strength play-prior factor]
 (defm calc-payoff [player p1-hand p1-action p2-hand p2-action]
  ;; Calculate payoff given actions and hands.  Pay outs are not symmetric 
  ;; due to the blinds
  (case p1-action
   :fold (if (= player 1) -1 1) ;; Pick up small blinds
   :bet (case p2-action
         :fold (if (= player 1) 2 -2) ;; Pick up big blinds
         :bet (case [player (> p2-hand p1-hand)] ;; Showdown
	           [1 true] -6 [1 false] 6 [2 true] 6 [2 false] -6))))
	
 (defm payoff-metric [payoff]
  ;; Hueristic model converting a payoff to a log score
  (* 3 (log (/ (+ payoff 6) 12))))
	
 (defquery p2-sim [p2-hand p1-action]
  ;; Simulator for player 2 who know's player 1's action but not his
  ;; hand.  Returns action
  (let [p2-action (sample (play-prior p2-hand))
        p1-hand (sample (hand-strength))] ;; Simulate a hand for player 1
   (observe (play-prior p1-hand) p1-action) ;; Condition on known action
   (observe (factor) ;; Factor trace probability with payoff metric
    (payoff-metric (calc-payoff 2 p1-hand p1-action p2-hand p2-action)))
   p2-action)) ;; Return action
	
 (defquery p1-sim [p1-hand M]
  ;; Simulator for player 1 who reasons about what player 2
  ;; might do to choose an action given a hand
  (let [p1-action (sample (play-prior p1-hand)) ;; Sample action
        p2-hand (sample (hand-strength)) ;; Sample hand for opponent
        p2-dist (conditional p2-sim :smc :number-of-particles M)
        p2-action (if (= p1-action :fold)
                      :bet ;; No need to simulate player 2
                      (sample (p2-dist p2-hand p1-action)))] 
   (observe (factor) ;; Factor trace probability with payoff metric
   (payoff-metric (calc-payoff 1 p1-hand p1-action p2-hand p2-action)))
   [p1-action p2-action]))) ;; Return actions
	
(defn estimate-actions [hand M]
 ;; Estimates the relative probability of betting for a hand
 (->> (doquery :importance p1-sim [hand M])
      (take 10000) collect-results empirical-distribution))
	\end{lstlisting}
	\vspace{-10pt}
	\caption{Code simulating the behavior of a poker player who reasons about the behavior of another player.
		Explanation provided in text.\label{fig:poker-code}}
\end{figure}

The two key functions here are the queries \clj{p1-sim} and \clj{p2-sim}, representing simulators for the two
players.  The simulations for each player exploit a utility function, which is a deterministic function of
the two hands and actions taken, to reflect the preference for actions which give a bigger return.
P1 acts before P2 and must thus not only reason about what hands P2 might
have, but also the actions P2 might take.  To do this, P1 utilizes the simulation for P2,
which takes in as inputs an observed action from P1 and a true hand for P2, returning actions taken
by P2.  P2 has incomplete information -- he does not know P1's hand -- and so the simulation of P2's action
requires inference, with a normalization constant that depends on P2's hand and P1's action, both of which
are random variables in the outer query \clj{p1-sim}.  This therefore corresponds to the nested sampling class
of nested estimation problems.

\begin{figure*}[t!]
	\centering
	\begin{subfigure}[b]{0.47\textwidth}
		\centering
		\includegraphics[width=\textwidth,trim={1.5cm 0 3.5cm 0},clip]{poker1}
		\caption{Probability player 1 betting \label{fig:poker1}}
	\end{subfigure}
	~~
	\begin{subfigure}[b]{0.47\textwidth}
		\centering
		\includegraphics[width=\textwidth,trim={1.5cm 0 3.5cm 0},clip]{poker2}
		\caption{Probability player 2 betting\label{fig:poker2}}
	\end{subfigure}
	\vspace{-6pt}
	\caption{Probabilities of each player betting output by \clj{p1-sim} for different computational budgets of the inner
		estimator.  The ostensibly strange behavior that P2 is more likely to bet as the strength of P1 hand's
		increases is because \clj{p1-sim} conditions on having a good return for P1 and when P1 has a good hand,
		it becomes increasingly beneficial for that bet to be called.  In other words, (b) is explicitly not the 
		marginal distribution for optimal betting of P2 which would require a separate calculation.  
		\label{fig:poker-line}\vspace{-10pt}}
\end{figure*}	

Keen eyed readers may have noticed that this use of \conditional in \clj{p1-sim} is distinct to elsewhere in
the paper as we have explicitly used SMC inference with a provided number of particles $M$ for \conditional.  This provides a
roundabout means of controlling the computational budget for calls to \conditional, as we showed is required for convergence in
Section~\ref{sec:samp}.  In Figure~\ref{fig:poker-line} we see that changing $M$ changes the probability
of each player betting under the model.  Increasing $M$ corresponds to P2's calculation being carried out more
carefully and so it is perhaps not surprising that it becomes less beneficial for P1 to bet with a weak hand as $M$
increases.  Nonetheless, even for a large $M$ it remains beneficial for P1 to bet with less than average hands, 
reflecting the fact that money is already invested in the pot through the blinds and the opportunity to win through
bluffing.

\subsubsection{Exact Sampling}
\label{sec:exact}

It may in fact be possible to provide consistent estimates in many nested query problems without requiring infinite computation
for each nested call by using exact sampling methods such as rejection sampling.
Such an approach is taken by Church~\citep{goodman2008church}, wherein no sample ever returns until it passes its 
local acceptance criterion.  Church is able to do this because it only allows for hard conditioning 
on events with non-zero measure, allowing it to take a guess-and-check process that produces an exact sample
in finite time by simply sampling from the generative model until the condition is satisfied.
Although the performance clearly
gets exponentially worse with increased nesting for such setups, this is a change in the constant factor of the
computation, not its scaling with the number of samples taken:
generating a single exact sample of the distribution has a finite expected time using rejection sampling which is thus
a constant factor in the convergence rate.

Unfortunately, most problems require conditioning on measure zero events because they include continuous data
-- they require a soft conditioning akin to the inclusion of a likelihood term -- and so cannot be tackled using Church.
Constructing a generic exact sampler for soft conditioning in an automated way is likely to be insurmountably problematic
in practice. Nonetheless, it does open up the intriguing prospect
of a hypothetical system that provides a standard Monte Carlo convergence rate for multiply-intractable distributions.
This assertion is a somewhat startling result: it suggests that Monte Carlo 
estimates made using nested exact sampling methods have a fundamentally different
convergence rate for nested inference problems (though not nested estimation problems in general) than, say,
nested self-normalized importance sampling (SNIS).  Amongst other things, this might lead, 
perhaps through combination with 
the work of~\cite{moller2006efficient}, to a contradiction of the, ostensibly reasonable, conjecture
made by~\cite{murray2004bayesian} that there are no generic tractable MCMC schemes for doubly-intractable distributions.
We leave formal analysis of this tantalizing line of inquiry to future work.
%It is beyond the scope of the work to analyze this hypothesis more formally, or the rabbit hole of
%nested exact sampling methods more generally, but we highlight that this constitutes a potentially fascinating line of inquiry.



\subsection{Nested Observation}
\label{sec:cond}


An alternative way one might wish to nest queries is through nested observation, whereby we
condition on the output of another query being a certain value.  For hard-constraints such
as used in Church, this is equivalent to query nesting through sampling.  However, for soft
constraints it can be substantially different.  The distinction is the same as between
\sample and \observe in Anglican -- we are observing an outcome of a program, rather than sampling
from it.  As \observe returns no outputs, the mathematical interpretation of observing 
the output of another query is that we are factoring the outer program trace weight by the
partition function estimate of the inner query.  Presuming that our partition function estimates
are unbiased, 
this corresponds to a particular instance of the products of expectations special case
and so we can directly apply Theorem~\ref{the:prod}.  It, therefore, follows that if
the outer estimator uses importance sampling or SMC, then such an approach is consistent through
proper weighting~\cite{naessethLS2015nested}.  More
generally, this case corresponds to a pseudo-marginal approach where the samples
from the inner estimator are never returned.  We can, therefore, use existing results, e.g.~\cite{andrieu2009pseudo},
to further demonstrate the consistency of the approach for other choices of outer estimator.
%For example, consistency when using SMC in the outer estimator follows directly
%from a combination of the consistency of the importance sampler and the results
%of~\cite{naessethLS2015nested}.
%It should also be possible to construct consistent approaches using MCMC samplers
%at the top level as per~\cite{andrieu2009pseudo}.

In addition to the statistical complications just discussed,
there are some significant semantic complications associated with nested conditioning.  
Though one may wish to simply run a nested query unmodified and factor the trace probability
by the partition function estimate, e.g. to construct a PMMH sampler~\cite{andrieu2010particle}
as done in~\cite{rainforth2016nips}, this is more of a means of
replacing an analytic likelihood term with an unbiased estimate, than a general purpose nested observation.
Instead, we might wish to estimate the likelihood of a query producing a particular output.
Unfortunately this is, in general, not possible for existing universal PPSs
because the density of the output variables are affected by deterministic computations in the query and
it is not usually possible to carry out the required change of variables computations automatically.
However, this problem is identical to 
that encountered in estimating the conditional marginal likelihood in~\cite{rainforth2016nips}
presenting an interesting possibility for constructing a nested observation statement -- one could use their
marginal program transformation to estimate the partition
function with certain \sample outputs ``clamped''.  
%, thereby constructing a similar scheme 
%to~\cite{rainforth2016bayesian} where the Bayesian optimization wrapper is replaced
%with an estimation scheme, i.e. the outer query.

\begin{figure}[t]
	\centering		
	\vspace{-6pt}
	\rule{\linewidth}{0.4pt}
	\vspace{-22pt}		
	\begin{lstlisting}[basicstyle=\ttfamily\footnotesize,multicols=2,frame=none]
(defm prior [] (normal 0 1))
(defm lik [theta d] (normal theta d))
	
(defquery inner-q [y d]
 (let [theta (sample (prior))]
  (observe (lik theta d) y)))
	
(defn inner-E [y d M]
 (->> (doquery :importance inner-q [y d])
      (take M)
      log-marginal))
	
	
(with-primitive-procedures [inner-E]
 (defquery outer-q [d M]
  (let [theta (sample (prior))
        y (sample (lik theta d))
        log-lik (observe* (lik theta d) y)
        log-marg (inner-E y d M)]
   (- log-lik log-marg))))
	
 (defn outer-E [d M N]
  (->> (doquery :importance outer-q [d M])
       (take N)
       collect-results
       empirical-mean))
	\end{lstlisting}
	\vspace{-14pt}		
	\rule{\linewidth}{0.4pt}
	%\vspace{5pt}
	\caption{Anglican code for Bayesian experimental design.
		%	    corresponding to the estimator
		%		given in~\eqref{eq:exp-des-nmc}.  
		By changing the definitions of \clj{prior}
		and \clj{lik}, this code can be used as a
		NMC estimator (consistent as $N,M\rightarrow\infty$) for any static
		Bayesian experimental design problem.
		Here \lsi{observe*} is a function for returning the log likelihood (it does not
		affect the trace probability), \lsi{log-marginal} produces a marginal likelihood estimated
		from a collection of weighted samples,
		and \lsi{->>} successively applies a series of functions calls,
		using the result of one as the last input the next.  When \lsi{outer-E} is invoked,
		this runs importance sampling on \lsi{outer-q}, which, in addition to carrying out
		its own computation, calls \lsi{inner-E}.  This in turn invokes another inference over
		\lsi{inner-q}, such that a \mc estimate using \lsi{M} samples is constructed for
		each sample of \lsi{outer-q}.  Thus \lsi{log-marg} is the \mc estimate itself.
		The final returned value is the (weighted) empirical mean for
		the outputs of \lsi{outer-q}. 
		%\vspace{-8pt}
		\label{fig:nest:exp}}	
\end{figure}

\subsection{Estimates as Variables}
\label{sec:var}


Finally, one might wish to use estimates as first class variables in another query.  In our previous examples,
nonlinear usage of expectations only ever manifested through inversion of the normalization
constant.  These methods are therefore clearly insufficient for expressing more general
nested estimation problems as would be required by, for example, experimental design.
%One can implicitly use expectation estimates as first class variables in Anglican 
%by either calling \doquery inside a \defdist deceleration or in a \defn function
%passed to a query using \clj{with-primitive-procedures}.  
An example of this is shown
in Figure~\ref{fig:nest:exp} corresponding to a generic program for carrying out Bayesian experimental
design~\citep{chaloner1995bayesian}.  The validity of this ``estimates as variables'' 
problem class is effectively
equivalent to that of NMC more generally and needs to be considered on a case-by-case basis. 


